ZipIt! Merging Models from Different Tasks without Training

Typical deep visual recognition models are capable of performing the one task they were trained on. In this paper, we tackle the extremely difficult problem of combining distinct models with different initializations, each solving a separate task, into one multi-task model without any additional training. Prior work in model merging permutes one model to the space of the other then averages them together. While this works for models trained on the same task, we find that this fails to account for the differences in models trained on disjoint tasks. Thus, we introduce "ZipIt!", a general method for merging two arbitrary models of the same architecture that incorporates two simple strategies. First, in order to account for features that aren't shared between models, we expand the model merging problem to allow for merging features within each model by defining a general "zip" operation. Second, we add support for partially zipping the models up until a specified layer, naturally creating a multi-head model. We find that these two changes combined account for 20-60% improvement over prior work, making it more feasible to merge models trained on disjoint tasks without retraining.

==> figures/14_model_size.tex <==
% \begin{wrapfigure}{l}{0.48\linewidth}
% % \begin{figure}[t]
% \centering
% %
% \begin{center}
%     \includegraphics[width=0.95\linewidth]{figures/imgs/model_scale.png}
% \end{center}
% \caption{{\bf Model Scale.} As we increase the width of the ResNet-20 models used for the CIFAR-100 (50+50) setting, \name{}\ makes effective use of that extra capacity, quickly approaching ensemble accuracy. 
% Git Re-Basin \cite{ainsworth2022git} and Permute only slightly benefit from the extra scale.
% }
% \label{fig:model_size}
% \end{wrapfigure}
% % \end{figure}

==> figures/1_capabilities_DEL.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/imgs/vs_prior_work.png}
%     \caption{{\bf Our Setting.} Prior work \cite{wortsman2022model,ainsworth2022git,jordan2022repair}
%     focuses on merging models from the \modelb{\textbf{same} dataset} with the \modelb{\textbf{same} label sets}: e.g., merging two models both trained to classify dog breeds. In this work, we remove that restriction and ``zip'' models that can come from \modela{\textbf{different} datasets} and have \modela{\textbf{different} label sets}: e.g., merging a model that classifies dog breeds with one that classifies bird species.
%     }
%     \label{fig:capabilities}
% \end{figure}

==> figures/5_partial_zip_DEL.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/imgs/partial_zip.png}
%     \caption{
%         {\bf Partial Zip.} 
%         If we stop zipping early (a), we can create a multi-head model that can perform multiple tasks. All we need to do is apply the last unmerge from zip propogation (Fig.~\ref{fig:zip_prop}) to the inputs of the first unmerged layer in each model (b), and we get a model with multiple heads (c).
%     }
%     \label{fig:partial_zip}
% \end{figure}

==> figures/A5_cifar_logits.tex <==

%##################################################################################################
\begin{table*}[t]
\centering
\subfloat[
    \textbf{CIFAR-10 (5+5)} VGG11 ($1\times$ width).
    \label{tab:cifar5+5}
]{
\centering
\begin{minipage}{0.47\linewidth}{
\begin{center}
\resizebox{\textwidth}{!}{
    \tablestyle{5pt}{1.1}
\begin{tabular}{y{53}x{40}|x{30}x{30}x{30}x{30}}
    & & \multicolumn{4}{c}{Accuracies (\%)}\\
    Method & FLOPs (G) & Joint & \modela{Task A} & \modelb{Task B} & Avg \\
    \shline
    \modela{Model A}                        & {0.15} & {44.6\conf{1.0}} & {89.2\conf{2.0}} & {21.0\conf{1.5}} & {55.1\conf{1.5}} \\
    \modelb{Model B}                        & {0.15} & {44.0\conf{1.4}} & {23.1\conf{4.5}} & {88.1\conf{2.8}} & {55.6\conf{3.4}} \\
    \hline
    W. Avg                                  &  0.15     & {10.2\conf{0.2}}           & {20.8\conf{1.2}}           & {20.9\conf{0.7}}           & {20.9\conf{0.7}} \\
    Permute                                 &  0.15     & {25.4\conf{1.1}}          & {47.2\conf{1.3}}          & {48.5\conf{12.3}}          & {47.8\conf{5.8}} \\
    \default{{\bf \name{}}$_\text{22/22}$}  &  0.15     & \textbf{33.2\conf{9.3}}   & \textbf{53.8\conf{14.7}}   & \textbf{59.9\conf{9.6}}   & \textbf{56.5\conf{6.5}} \\
    \hline
    \gc{Ensemble}                           & \gc{0.30} & \gc{66.6\conf{2.5}}       & \gc{89.2\conf{2.0}}       & \gc{88.1\conf{2.8}}       &  \gc{88.6\conf{0.5}} \\
    \default{{\bf \name{}}$_\text{14/22}$}  & {0.17}    & {35.2\conf{6.0}}          & {56.7\conf{13.7}}          & {60.2\conf{15.9}}          & {58.4\conf{5.9}} \\
    \default{{\bf \name{}}$_\text{7/22}$}   & {0.27}    &  \textbf{44.5\conf{2.9}}  &  \textbf{66.0\conf{4.2}}    & \textbf{65.1\conf{11.2}} & \textbf{65.5\conf{4.1}} \\
\end{tabular}
}
\end{center}
}\end{minipage}
}
\hspace{1em}
\centering
\subfloat[
    \textbf{CIFAR-100 (50+50).} ResNet-20 (16$\times$ width).
    \label{tab:cifar50+50}
]{
\centering
\begin{minipage}{0.47\linewidth}{
\begin{center}
\resizebox{\textwidth}{!}{
    \tablestyle{5pt}{1.1}
\begin{tabular}{y{53}x{40}|x{30}x{30}x{30}x{30}}
        & & \multicolumn{4}{c}{Accuracies (\%)}\\
        Method & FLOPs (G) & Joint & \modela{Task A} & \modelb{Task B} & Avg \\
    \shline
    \modela{Model A}                        & {10.88} & {37.9\conf{0.2}} & {74.15\conf{0.6}} & {1.7\conf{0.3}} & {36.4\conf{0.7}} \\
    \modelb{Model B}                        & {10.88} & {36.7\conf{1.2}} & {2.2\conf{0.5}} & {75.2\conf{2.3}} & {38.7\conf{1.1}} \\
    \hline
    W. Avg                                  &  10.88     & {2.7\conf{0.1}}           & {5.0\conf{3.3}}           & {4.9\conf{1.2}}           & {4.9\conf{0.1}} \\
    Git Re-Basin$\ddag$                     &  10.88     & {3.1\conf{0.8}}           & {5.8\conf{0.9}}           & {5.3\conf{0.8}}           & {5.6\conf{0.8}}  \\
    Permute                                 &  10.88     & {20.0\conf{1.3}}          & {30.8\conf{3.3}}          & {32.8\conf{1.6}}          & {31.8\conf{1.7}} \\
    \default{{\bf \name{}}$_\text{20/20}$}  &  10.88     & \textbf{27.9\conf{1.5}}   & \textbf{40.1\conf{2.4}}   & \textbf{39.7\conf{1.6}}   & \textbf{39.9\conf{1.9}} \\
    \hline
    \gc{Ensemble}                           & \gc{21.76} & \gc{60.5\conf{1.0}}       & \gc{74.2\conf{0.6}}       & \gc{75.2\conf{2.3}}       &  \gc{74.7\conf{1.4}} \\
    \default{{\bf \name{}}$_\text{13/20}$}  & {14.52}    & {38.6\conf{2.4}}          & {51.8\conf{1.6}}          & {52.0\conf{3.5}}          & {51.9\conf{2.4}} \\
    \default{{\bf \name{}}$_\text{7/20}$}   & {18.14}    &  \textbf{47.0\conf{2.2}}         &  \textbf{60.6\conf{1.2}}         & \textbf{60.5\conf{3.2}}          & \textbf{60.6\conf{2.1}} \\
\end{tabular}
}
\end{center}
}\end{minipage}
}
\caption{\textbf{Cross Entropy Results.} \name{}\ vs. baselines across the architectures.
on combining a model trained on half the classes (\modela{Task A}) with one trained on the other half (\modelb{Task B}) \textit{without extra training}. We report both joint (10/100-way) and per-task (5/50-way) accuracy.
\name{}\ \textit{significantly} outperforms its baseline and closes in on the \gc{upper bound} (ensemble accuracy).
$\ddag$ refers to \cite{ainsworth2022git}
}
\label{tab:cifar_results}
\vspace{-15pt}
\end{table*}
